Sparse Multilevel Roadmaps for High-Dimensional Robot Motion Planning

Sparse roadmaps are important to compactly represent state spaces, to determine problems to be infeasible and to terminate in finite time. However, sparse roadmaps do not scale well to high-dimensional planning problems. In prior work, we showed improved planning performance on high-dimensional planning problems by using multilevel abstractions to simplify state spaces. In this work, we generalize sparse roadmaps to multilevel abstractions by developing a novel algorithm, the sparse multilevel roadmap planner (SMLR). To this end, we represent multilevel abstractions using the language of fiber bundles, and generalize sparse roadmap planners by using the concept of restriction sampling with visibility regions. We argue SMLR to be probabilistically complete and asymptotically near-optimal by inheritance from sparse roadmap planners. In evaluations, we outperform sparse roadmap planners on challenging planning problems, in particular problems which are high-dimensional, contain narrow passages or are infeasible. We thereby demonstrate sparse multilevel roadmaps as an efficient tool for feasible and infeasible high-dimensional planning problems.

==> images/pullfigure/pullfigure_small.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.48\linewidth}
        \vskip 0pt
        \includegraphics[width=\linewidth]{images/pullfigure/02D_torus_SPARStwo.png}
        \caption{Sparse roadmap on Torus $T^2=S^1\times S^1$ with $S^1$ being the circle. Generated using the sparse roadmap planner (SPARS) by Dobson and Bekris \cite{dobson_2014} using a uniform sampling distribution on $T^2$ \cite{Williamson1987}.}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.48\linewidth}
    \centering
        \vskip 0pt
        \includegraphics[width=\linewidth]{images/pullfigure/02D_torus_SMLR.png}
\begin{tikzpicture}[node distance=0.3cm]
\node [] (A) {};
\node [below=of A] (B) {};
\draw [-{Straight Barb}, fill=black, line width=0.5mm] (A) -- (B);
\end{tikzpicture}\\
        \includegraphics[width=0.65\textwidth]{images/pullfigure/02D_torus_SMLR_level0.png}
        \caption{Sparse multilevel roadmap on a path restriction over the fiber bundle $T^2 \rightarrow S^1$ generated using our method.}
    \end{subfigure}
    \caption{We generalize sparse roadmaps (left) to multilevel abstractions (right).}
\end{figure}

==> images/systems_figure.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
    [
        squarednode/.style={rectangle, draw=gray!60, fill=gray!5, very thick, minimum width =12mm},
        graphnode/.style={minimum width=12mm},
        arrow/.style={->},
        darrow/.style={->, dashed}
    ]
        \def\ystart{5}
        \def\stepY{1}

        \def\posX{2}
        %%Xk spaces
        \node[squarednode] (XK) at (\posX,\ystart){$\X_{K}$};
        \node[squarednode] (XKK) at (\posX,3){$\X_{K-1}$};
        \node[] (DOTS) at (\posX,2){$\vdots$};
        \node[squarednode] (X1) at (\posX,1){$\X_1$};
        \draw[arrow] (XK.south)--(XKK.north) node[midway,left]{$\texttt{ProjectBase}$};
        \draw[arrow] (XKK.south)--(DOTS.north);
        \draw[arrow] (DOTS.south)--(X1.north);
        
        %%Pointer
        \node[squarednode] (Xcur) at (-0.25,3){$\Xcur$};
        \node[squarednode] (Xtop) at (-0.25,1){$\Xtop$};
        \draw[darrow] (Xcur.east)--(XKK.west) node[midway,above] {$\texttt{PTC}$};
        \draw[darrow] (Xtop.east)--(X1.west) node[midway,above] {$\texttt{Grow}$};
        
        %%Gk graphs
        \def\posG{3.5}
        \node[graphnode] (GK) at (\posG,\ystart){$\G_{K}$};
        \node[graphnode] (GKK) at (\posG,3){$\G_{K-1}$};
        \node[] (GDOTS) at (\posG,2){$\vdots$};
        \node[graphnode] (G1) at (\posG,1){$\G_1$};
        \draw[arrow] (XKK.east)--(GKK.west);
        \draw[arrow] (XK.east)--(GK.west);
        \draw[arrow] (X1.east)--(G1.west);
        \draw[arrow] (GKK.south)--(GDOTS.north);
        \draw[arrow] (GDOTS.south)--(G1.north);
        
        %%descriptions
        \draw[arrow] (GK.south)--(GKK.north) node[midway,right] {$\texttt{SampleBase}$};
    \end{tikzpicture}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

